Dysca: A Dynamic and Scalable Benchmark for Evaluating Perception Ability of LVLMs

Currently many benchmarks have been proposed to evaluate the perception ability of the Large Vision-Language Models (LVLMs). However, most benchmarks conduct questions by selecting images from existing datasets, resulting in the potential data leakage. Besides, these benchmarks merely focus on evaluating LVLMs on the realistic style images and clean scenarios, leaving the multi-stylized images and noisy scenarios unexplored. In response to these challenges, we propose a dynamic and scalable benchmark named Dysca for evaluating LVLMs by leveraging synthesis images. Specifically, we leverage Stable Diffusion and design a rule-based method to dynamically generate novel images, questions and the corresponding answers. We consider 51 kinds of image styles and evaluate the perception capability in 20 subtasks. Moreover, we conduct evaluations under 4 scenarios (i.e., Clean, Corruption, Print Attacking and Adversarial Attacking) and 3 question types (i.e., Multi-choices, True-or-false and Free-form). Thanks to the generative paradigm, Dysca serves as a scalable benchmark for easily adding new subtasks and scenarios. A total of 24 advanced open-source LVLMs and 2 close-source LVLMs are evaluated on Dysca, revealing the drawbacks of current LVLMs. The benchmark is released at https://github.com/Robin-WZQ/Dysca.

==> leaderboard_o.tex <==


% \begin{table*}[h]
% \centering
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 80.13 \\
% 2    & InstructBlip       & 72.36 \\
% 3    & Blip2              & 70.03 \\
% 4    & Shikra-VQA         & 64.03 \\
% 5    & Shikra             & 62.97 \\
% 6    & Otter              & 62.22 \\
% 7    & Qwen-VL-Chat       & 61.13 \\
% 8    & LLAVA-1.5-13B      & 60.17 \\
% 9    & LLAVA-1.5-7B       & 53.81 \\
% 10   & MiniGPT-4          & 42.52 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Movie}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 95.89 \\
% 2    & InstructBlip       & 95.44 \\
% 3    & Blip2              & 94.64 \\
% 4    & Shikra-VQA         & 88.25 \\
% 5    & Qwen-VL-Chat       & 79.75 \\
% 6    & Shikra             & 77.65 \\
% 7    & Otter              & 69.10 \\
% 8    & LLAVA-1.5-13B      & 68.82 \\
% 9    & LLAVA-1.5-7B       & 62.77 \\
% 10   & MiniGPT-4          & 46.98 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Action}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 75.55 \\
% 2    & InstructBlip       & 63.42 \\
% 3    & Otter              & 63.04 \\
% 4    & Shikra-VQA         & 60.10 \\
% 5    & Blip2              & 59.14 \\
% 6    & Shikra             & 58.55 \\
% 7    & Qwen-VL-Chat       & 58.27 \\
% 8    & LLAVA-1.5-13B      & 56.69 \\
% 9    & LLAVA-1.5-7B       & 53.48 \\
% 10   & MiniGPT-4          & 40.23 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-TV Show}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 79.92 \\
% 2    & InstructBlip       & 77.84 \\
% 3    & Blip2              & 76.88 \\
% 4    & Shikra             & 73.55 \\
% 5    & Shikra-VQA         & 73.07 \\
% 6    & Qwen-VL-Chat       & 65.12 \\
% 7    & LLAVA-1.5-13B      & 62.86 \\
% 8    & Otter              & 60.95 \\
% 9    & LLAVA-1.5-7B       & 57.74 \\
% 10   & MiniGPT-4          & 42.06 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Profession}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & InstructBlip       & 96.90 \\
% 2    & Blip2              & 96.64 \\
% 3    & XComposer-VL & 96.43 \\
% 4    & Shikra-VQA         & 82.85 \\
% 5    & Shikra             & 80.17 \\
% 6    & Qwen-VL-Chat       & 75.84 \\
% 7    & LLAVA-1.5-13B      & 75.12 \\
% 8    & LLAVA-1.5-7B       & 69.74 \\
% 9    & Otter              & 62.50 \\
% 10   & MiniGPT-4          & 52.81 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Landmark}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 75.00 \\
% 2    & Qwen-VL-Chat       & 63.11 \\
% 3    & InstructBlip       & 62.66 \\
% 4    & Otter              & 59.56 \\
% 5    & Blip2              & 59.50 \\
% 6    & LLAVA-1.5-13B      & 53.88 \\
% 7    & Shikra-VQA         & 53.31 \\
% 8    & Shikra             & 52.84 \\
% 9    & LLAVA-1.5-7B       & 47.80 \\
% 10   & MiniGPT-4          & 38.98 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Anime}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 85.96 \\
% 2    & InstructBlip       & 83.80 \\
% 3    & Blip2              & 78.09 \\
% 4    & Shikra-VQA         & 69.83 \\
% 5    & Qwen-VL-Chat       & 69.58 \\
% 6    & Shikra             & 67.43 \\
% 7    & LLAVA-1.5-13B      & 61.20 \\
% 8    & Otter              & 58.33 \\
% 9    & LLAVA-1.5-7B       & 48.80 \\
% 10   & MiniGPT-4          & 40.86 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Clothes}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 87.91 \\
% 2    & InstructBlip       & 79.91 \\
% 3    & Blip2              & 79.23 \\
% 4    & Qwen-VL-Chat       & 68.71 \\
% 5    & Shikra-VQA         & 62.93 \\
% 6    & Shikra             & 61.81 \\
% 7    & LLAVA-1.5-13B      & 59.04 \\
% 8    & LLAVA-1.5-7B       & 56.04 \\
% 9    & Otter              & 52.97 \\
% 10   & MiniGPT-4          & 39.13 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Celebrity}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 91.27 \\
% 2    & InstructBlip       & 90.28 \\
% 3    & Blip2              & 89.78 \\
% 4    & Shikra-VQA         & 80.23 \\
% 5    & Shikra             & 75.84 \\
% 6    & Qwen-VL-Chat       & 71.37 \\
% 7    & LLAVA-1.5-13B      & 68.16 \\
% 8    & Otter              & 63.22 \\
% 9    & LLAVA-1.5-7B       & 52.87 \\
% 10   & MiniGPT-4          & 47.72 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Food}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 93.19 \\
% 2    & InstructBlip       & 92.62 \\
% 3    & Blip2              & 91.84 \\
% 4    & Shikra-VQA         & 80.05 \\
% 5    & Shikra             & 77.57 \\
% 6    & Qwen-VL-Chat       & 76.11 \\
% 7    & Otter              & 73.96 \\
% 8    & LLAVA-1.5-13B      & 67.61 \\
% 9    & LLAVA-1.5-7B       & 48.84 \\
% 10   & MiniGPT-4          & 47.95 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Plant}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 73.12 \\
% 2    & InstructBlip       & 62.34 \\
% 3    & Shikra-VQA         & 61.42 \\
% 4    & Blip2              & 61.13 \\
% 5    & Shikra             & 61.04 \\
% 6    & LLAVA-1.5-13B      & 54.57 \\
% 7    & Qwen-VL-Chat       & 51.28 \\
% 8    & LLAVA-1.5-7B       & 46.75 \\
% 9    & Otter              & 44.58 \\
% 10   & MiniGPT-4          & 41.73 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Age}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 98.83 \\
% 2    & Blip2              & 97.12 \\
% 3    & InstructBlip       & 93.86 \\
% 4    & LLAVA-1.5-13B      & 91.12 \\
% 5    & Shikra-VQA         & 90.40 \\
% 6    & Shikra             & 85.50 \\
% 7    & Qwen-VL-Chat       & 78.13 \\
% 8    & Otter              & 78.09 \\
% 9    & MiniGPT-4          & 52.86 \\
% 10   & LLAVA-1.5-7B       & 51.96 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Gender}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%        1    & XComposer-VL & 86.08 \\
% 2    & InstructBlip       & 85.59 \\
% 3    & Shikra-VQA         & 83.53 \\
% 4    & Blip2              & 82.59 \\
% 5    & Shikra             & 80.51 \\
% 6    & Qwen-VL-Chat       & 74.76 \\
% 7    & Otter              & 67.11 \\
% 8    & LLAVA-1.5-13B      & 64.81 \\
% 9    & LLAVA-1.5-7B       & 56.81 \\
% 10   & MiniGPT-4          & 46.46 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Expression}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 78.56 \\
% 2    & InstructBlip       & 76.31 \\
% 3    & Blip2              & 73.16 \\
% 4    & LLAVA-1.5-13B      & 66.50 \\
% 5    & Qwen-VL-Chat       & 65.19 \\
% 6    & Shikra-VQA         & 64.56 \\
% 7    & Shikra             & 64.53 \\
% 8    & Otter              & 50.44 \\
% 9    & LLAVA-1.5-7B       & 47.27 \\
% 10   & MiniGPT-4          & 38.98 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Race}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%       1    & XComposer-VL & 97.27 \\
% 2    & InstructBlip       & 96.09 \\
% 3    & Blip2              & 95.95 \\
% 4    & Shikra-VQA         & 82.72 \\
% 5    & Otter              & 82.47 \\
% 6    & Qwen-VL-Chat       & 79.98 \\
% 7    & Shikra             & 79.44 \\
% 8    & LLAVA-1.5-13B      & 72.11 \\
% 9    & LLAVA-1.5-7B       & 50.08 \\
% 10   & MiniGPT-4          & 47.77 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Animal}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%        1    & XComposer-VL & 90.97 \\
% 2    & InstructBlip       & 90.00 \\
% 3    & Blip2              & 88.53 \\
% 4    & Shikra-VQA         & 82.72 \\
% 5    & Qwen-VL-Chat       & 75.73 \\
% 6    & Shikra             & 70.06 \\
% 7    & LLAVA-1.5-13B      & 67.89 \\
% 8    & Otter              & 64.91 \\
% 9    & LLAVA-1.5-7B       & 54.31 \\
% 10   & MiniGPT-4          & 51.65 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Object}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & Blip2              & 68.38 \\
% 2    & InstructBlip       & 67.50 \\
% 3    & XComposer-VL & 66.06 \\
% 4    & Shikra-VQA         & 64.86 \\
% 5    & Otter              & 64.37 \\
% 6    & Qwen-VL-Chat       & 63.28 \\
% 7    & Shikra             & 63.02 \\
% 8    & LLAVA-1.5-13B      & 58.84 \\
% 9    & LLAVA-1.5-7B       & 44.96 \\
% 10   & MiniGPT-4          & 43.70 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-OCR}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 73.94 \\
% 2    & Blip2              & 66.98 \\
% 3    & InstructBlip       & 66.77 \\
% 4    & Otter              & 63.82 \\
% 5    & Qwen-VL-Chat       & 61.80 \\
% 6    & Shikra             & 57.21 \\
% 7    & Shikra-VQA         & 56.89 \\
% 8    & LLAVA-1.5-13B      & 55.68 \\
% 9    & LLAVA-1.5-7B       & 49.05 \\
% 10   & MiniGPT-4          & 41.47 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Style}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL & 73.27 \\
% 2    & Shikra-VQA         & 68.47 \\
% 3    & InstructBlip       & 67.84 \\
% 4    & Shikra             & 66.95 \\
% 5    & Blip2              & 66.17 \\
% 6    & Otter              & 63.23 \\
% 7    & Qwen-VL-Chat       & 60.51 \\
% 8    & LLAVA-1.5-13B      & 59.00 \\
% 9    & LLAVA-1.5-7B       & 47.64 \\
% 10   & MiniGPT-4          & 41.02 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Background}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL & 88.50 \\
% 2    & InstructBlip       & 88.24 \\
% 3    & Blip2              & 86.78 \\
% 4    & Shikra-VQA         & 74.14 \\
% 5    & Shikra             & 73.37 \\
% 6    & Qwen-VL-Chat       & 69.72 \\
% 7    & LLAVA-1.5-13B      & 58.36 \\
% 8    & Otter              & 53.12 \\
% 9    & LLAVA-1.5-7B       & 46.91 \\
% 10   & MiniGPT-4          & 42.90 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Clean-Color}}
% \end{minipage}
% \vspace{0.1cm}
% \caption{Leaderboards of all Perceptual tasks under clean scenario.}
% \label{leaderboard_clean_fine_grain}
% \end{table*}

% % ================================================================================================================

% \begin{table*}[h]
% \centering
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 78.20  \\
% 2    & InstructBlip              & 71.30  \\
% 3    & Blip2                     & 68.69 \\
% 4    & Shikra-VQA                & 64.19 \\
% 5    & Shikra                    & 63.47 \\
% 6    & Otter                     & 61.39 \\
% 7    & Qwen-VL                   & 59.27 \\
% 8    & LLAVA-1.5-13B             & 58.67 \\
% 9    & LLAVA-1.5-7B              & 52.36 \\
% 10   & MiniGPT-4                 & 43.02 \\

%         \end{tabular}
%     }
    
%     \subcaption{\textit{Corru.-Movie}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 95.86 \\
% 2    & InstructBlip              & 95.09 \\
% 3    & Blip2                     & 93.87 \\
% 4    & Shikra-VQA                & 88.72 \\
% 5    & Shikra                    & 77.77 \\
% 6    & Qwen-VL                   & 75.09 \\
% 7    & Otter                     & 70.09 \\
% 8    & LLAVA-1.5-13B             & 68.34 \\
% 9    & LLAVA-1.5-7B              & 63.00 \\
% 10   & MiniGPT-4                 & 47.22 \\


%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Action}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 72.86 \\
% 2    & InstructBlip              & 62.42 \\
% 3    & Otter                     & 60.71 \\
% 4    & Shikra                    & 60.09 \\
% 5    & Shikra-VQA                & 59.58 \\
% 6    & Blip2                     & 58.16 \\
% 7    & Qwen-VL                   & 57.95 \\
% 8    & LLAVA-1.5-13B             & 55.18 \\
% 9    & LLAVA-1.5-7B              & 52.34 \\
% 10   & MiniGPT-4                 & 38.70 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-TV Show}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 78.48 \\
% 2    & InstructBlip              & 77.84 \\
% 3    & Blip2                     & 75.77 \\
% 4    & Shikra                    & 73.72 \\
% 5    & Shikra-VQA                & 73.38 \\
% 6    & Qwen-VL                   & 64.97 \\
% 7    & Otter                     & 62.71 \\
% 8    & LLAVA-1.5-13B             & 62.23 \\
% 9    & LLAVA-1.5-7B              & 56.95 \\
% 10   & MiniGPT-4                 & 43.22 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Profession}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & InstructBlip              & 96.33 \\
% 2    & Blip2                     & 96.28 \\
% 3    & XComposer-VL              & 95.97 \\
% 4    & Shikra-VQA                & 83.01 \\
% 5    & Shikra                    & 82.38 \\
% 6    & LLAVA-1.5-13B             & 74.63 \\
% 7    & Qwen-VL                   & 73.55 \\
% 8    & LLAVA-1.5-7B              & 68.78 \\
% 9    & Otter                     & 61.65 \\
% 10   & MiniGPT-4                 & 49.55 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Landmark}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 72.28 \\
% 2    & InstructBlip              & 62.79 \\
% 3    & Qwen-VL                   & 60.44 \\
% 4    & Blip2                     & 58.67 \\
% 5    & Otter                     & 57.24 \\
% 6    & LLAVA-1.5-13B             & 53.67 \\
% 7    & Shikra-VQA                & 52.28 \\
% 8    & Shikra                    & 52.00 \\
% 9    & LLAVA-1.5-7B              & 47.87 \\
% 10   & MiniGPT-4                 & 40.91 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Anime}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 84.87 \\
% 2    & InstructBlip              & 82.84 \\
% 3    & Blip2                     & 76.69 \\
% 4    & Shikra-VQA                & 70.59 \\
% 5    & Shikra                    & 67.05 \\
% 6    & Qwen-VL                   & 64.26 \\
% 7    & LLAVA-1.5-13B             & 60.88 \\
% 8    & Otter                     & 59.87 \\
% 9    & LLAVA-1.5-7B              & 48.12 \\
% 10   & MiniGPT-4                 & 41.38 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Clothes}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 87.25 \\
% 2    & InstructBlip              & 79.23 \\
% 3    & Blip2                     & 78.36 \\
% 4    & Qwen-VL                   & 64.89 \\
% 5    & Shikra-VQA                & 62.55 \\
% 6    & Shikra                    & 61.68 \\
% 7    & LLAVA-1.5-13B             & 58.64 \\
% 8    & LLAVA-1.5-7B              & 56.36 \\
% 9    & Otter                     & 53.59 \\
% 10   & MiniGPT-4                 & 38.80 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Celebrity}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 90.61 \\
% 2    & InstructBlip              & 90.08 \\
% 3    & Blip2                     & 89.19 \\
% 4    & Shikra-VQA                & 80.55 \\
% 5    & Shikra                    & 75.63 \\
% 6    & Qwen-VL                   & 70.71 \\
% 7    & LLAVA-1.5-13B             & 67.46 \\
% 8    & Otter                     & 65.06 \\
% 9    & LLAVA-1.5-7B              & 52.94 \\
% 10   & MiniGPT-4                 & 47.76 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Food}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 92.45 \\
% 2    & InstructBlip              & 92.23 \\
% 3    & Blip2                     & 91.15 \\
% 4    & Shikra-VQA                & 80.80 \\
% 5    & Shikra                    & 77.69 \\
% 6    & Otter                     & 73.42 \\
% 7    & Qwen-VL                   & 72.01 \\
% 8    & LLAVA-1.5-13B             & 67.22 \\
% 9    & LLAVA-1.5-7B              & 48.84 \\
% 10   & MiniGPT-4                 & 48.04 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Plant}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 73.04 \\
% 2    & InstructBlip              & 61.59 \\
% 3    & Shikra-VQA                & 61.09 \\
% 4    & Shikra                    & 60.40 \\
% 5    & Blip2                     & 60.03 \\
% 6    & Qwen-VL                   & 55.26 \\
% 7    & LLAVA-1.5-13B             & 53.67 \\
% 8    & LLAVA-1.5-7B              & 46.76 \\
% 9    & Otter                     & 45.09 \\
% 10   & MiniGPT-4                 & 40.84 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Age}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 98.53 \\
% 2    & Blip2                     & 97.76 \\
% 3    & InstructBlip              & 93.75 \\
% 4    & LLAVA-1.5-13B             & 91.09 \\
% 5    & Shikra-VQA                & 90.17 \\
% 6    & Shikra                    & 85.91 \\
% 7    & Otter                     & 80.22 \\
% 8    & Qwen-VL                   & 67.00 \\
% 9    & MiniGPT-4                 & 52.75 \\
% 10   & LLAVA-1.5-7B              & 52.27 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Gender}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 86.24 \\
% 2    & InstructBlip              & 84.95 \\
% 3    & Shikra-VQA                & 83.56 \\
% 4    & Blip2                     & 81.56 \\
% 5    & Shikra                    & 80.56 \\
% 6    & Qwen-VL                   & 70.55 \\
% 7    & Otter                     & 66.64 \\
% 8    & LLAVA-1.5-13B             & 64.94 \\
% 9    & LLAVA-1.5-7B              & 56.16 \\
% 10   & MiniGPT-4                 & 46.55 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Expression}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 78.80 \\
% 2    & InstructBlip              & 76.19 \\
% 3    & Blip2                     & 71.72 \\
% 4    & LLAVA-1.5-13B             & 65.33 \\
% 5    & Shikra-VQA                & 64.73 \\
% 6    & Shikra                    & 63.94 \\
% 7    & Qwen-VL                   & 63.55 \\
% 8    & Otter                     & 49.73 \\
% 9    & LLAVA-1.5-7B              & 47.92 \\
% 10   & MiniGPT-4                 & 39.65 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Race}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 97.06 \\
% 2    & InstructBlip              & 95.86 \\
% 3    & Blip2                     & 95.69 \\
% 4    & Shikra-VQA                & 83.03 \\
% 5    & Otter                     & 82.84 \\
% 6    & Shikra                    & 79.44 \\
% 7    & LLAVA-1.5-13B             & 71.47 \\
% 8    & Qwen-VL                   & 71.43 \\
% 9    & LLAVA-1.5-7B              & 50.67 \\
% 10   & MiniGPT-4                 & 48.66 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Animal}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 90.81 \\
% 2    & InstructBlip              & 89.76 \\
% 3    & Blip2                     & 88.05 \\
% 4    & Shikra-VQA                & 82.76 \\
% 5    & Shikra                    & 71.49 \\
% 6    & Qwen-VL                   & 67.78 \\
% 7    & LLAVA-1.5-13B             & 67.23 \\
% 8    & Otter                     & 66.18 \\
% 9    & LLAVA-1.5-7B              & 54.09 \\
% 10   & MiniGPT-4                 & 51.02 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Object}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Blip2                     & 94.06 \\
% 2    & InstructBlip              & 90.54 \\
% 3    & XComposer-VL              & 87.19 \\
% 4    & Shikra-VQA                & 80.80 \\
% 5    & Otter                     & 78.70 \\
% 6    & Shikra                    & 77.17 \\
% 7    & Qwen-VL                   & 69.66 \\
% 8    & LLAVA-1.5-13B             & 68.58 \\
% 9    & LLAVA-1.5-7B              & 49.10 \\
% 10   & MiniGPT-4                 & 44.63 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-OCR}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 72.34 \\
% 2    & InstructBlip              & 65.06 \\
% 3    & Blip2                     & 64.86 \\
% 4    & Otter                     & 61.14 \\
% 5    & Qwen-VL                   & 60.34 \\
% 6    & Shikra                    & 56.61 \\
% 7    & Shikra-VQA                & 55.81 \\
% 8    & LLAVA-1.5-13B             & 53.65 \\
% 9    & LLAVA-1.5-7B              & 47.67 \\
% 10   & MiniGPT-4                 & 40.81 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Courruption-Style}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 72.53 \\
% 2    & Shikra-VQA                & 68.25 \\
% 3    & InstructBlip              & 67.48 \\
% 4    & Shikra                    & 67.19 \\
% 5    & Blip2                     & 64.69 \\
% 6    & Otter                     & 62.99 \\
% 7    & Qwen-VL                   & 60.50 \\
% 8    & LLAVA-1.5-13B             & 58.50 \\
% 9    & LLAVA-1.5-7B              & 47.12 \\
% 10   & MiniGPT-4                 & 40.53 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Background}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 88.24 \\
% 2    & InstructBlip              & 88.09 \\
% 3    & Blip2                     & 86.25 \\
% 4    & Shikra-VQA                & 74.14 \\
% 5    & Shikra                    & 73.07 \\
% 6    & Qwen-VL                   & 70.78 \\
% 7    & LLAVA-1.5-13B             & 57.70 \\
% 8    & Otter                     & 56.14 \\
% 9    & LLAVA-1.5-7B              & 46.76 \\
% 10   & MiniGPT-4                 & 42.86 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.-Color}}
% \end{minipage}
% \vspace{0.1cm}
% \caption{Leaderboards of all Perceptual tasks under corruption scenario.}
% \label{leaderboard_corruption_fine_grain}
% \end{table*}


% % ================================================================================================================


% \begin{table*}[h]
% \centering
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 67.09 \\
% 2    & Blip2                     & 52.55 \\
% 3    & LLAVA-1.5-13B             & 46.74 \\
% 4    & LLAVA-1.5-7B              & 45.24 \\
% 5    & Shikra                    & 44.84 \\
% 6    & Shikra-VQA                & 44.36 \\
% 7    & Qwen-VL                   & 44.30 \\
% 8    & InstructBlip              & 43.06 \\
% 9    & MiniGPT-4                 & 40.26 \\
% 10   & Otter                     & 37.97 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Movie}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 86.24 \\
% 2    & Blip2                     & 79.13 \\
% 3    & InstructBlip              & 75.94 \\
% 4    & Shikra-VQA                & 71.36 \\
% 5    & Qwen-VL                   & 65.26 \\
% 6    & Shikra                    & 58.82 \\
% 7    & LLAVA-1.5-13B             & 57.66 \\
% 8    & LLAVA-1.5-7B              & 51.62 \\
% 9    & MiniGPT-4                 & 47.07 \\
% 10   & Otter                     & 39.77 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Action}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 55.08 \\
% 2    & LLAVA-1.5-7B              & 43.55 \\
% 3    & Qwen-VL                   & 40.72 \\
% 4    & LLAVA-1.5-13B             & 40.09 \\
% 5    & Blip2                     & 39.71 \\
% 6    & Shikra                    & 39.01 \\
% 7    & MiniGPT-4                 & 37.40 \\
% 8    & Shikra-VQA                & 36.50 \\
% 9    & InstructBlip              & 32.17 \\
% 10   & Otter                     & 31.48 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-TV Show}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 67.14 \\
% 2    & Blip2                     & 59.62 \\
% 3    & Shikra                    & 55.70 \\
% 4    & InstructBlip              & 54.52 \\
% 5    & Shikra-VQA                & 54.25 \\
% 6    & Qwen-VL                   & 48.66 \\
% 7    & LLAVA-1.5-13B             & 47.49 \\
% 8    & LLAVA-1.5-7B              & 42.86 \\
% 9    & MiniGPT-4                 & 42.22 \\
% 10   & Otter                     & 38.12 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Profession}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 89.81 \\
% 2    & Blip2                     & 84.85 \\
% 3    & InstructBlip              & 76.78 \\
% 4    & Shikra-VQA                & 68.28 \\
% 5    & LLAVA-1.5-13B             & 65.98 \\
% 6    & Shikra                    & 64.47 \\
% 7    & Qwen-VL                   & 64.29 \\
% 8    & LLAVA-1.5-7B              & 56.39 \\
% 9    & MiniGPT-4                 & 49.58 \\
% 10   & Otter                     & 43.89 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Landmark}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 59.72 \\
% 2    & Blip2                     & 45.05 \\
% 3    & Qwen-VL                   & 44.95 \\
% 4    & LLAVA-1.5-7B              & 42.23 \\
% 5    & LLAVA-1.5-13B             & 40.95 \\
% 6    & InstructBlip              & 38.26 \\
% 7    & Shikra-VQA                & 38.25 \\
% 8    & MiniGPT-4                 & 37.27 \\
% 9    & Shikra                    & 37.02 \\
% 10   & Otter                     & 36.16 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Anime}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 76.43 \\
% 2    & Blip2                     & 66.53 \\
% 3    & InstructBlip              & 62.14 \\
% 4    & Qwen-VL                   & 51.56 \\
% 5    & LLAVA-1.5-13B             & 49.63 \\
% 6    & Shikra-VQA                & 49.02 \\
% 7    & Shikra                    & 47.23 \\
% 8    & LLAVA-1.5-7B              & 42.22 \\
% 9    & MiniGPT-4                 & 39.66 \\
% 10   & Otter                     & 34.67 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Clothes}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 73.48 \\
% 2    & Blip2                     & 57.30 \\
% 3    & Qwen-VL                   & 52.34 \\
% 4    & LLAVA-1.5-7B              & 45.11 \\
% 5    & InstructBlip              & 43.36 \\
% 6    & Shikra                    & 43.13 \\
% 7    & Shikra-VQA                & 42.01 \\
% 8    & LLAVA-1.5-13B             & 41.59 \\
% 9    & MiniGPT-4                 & 38.64 \\
% 10   & Otter                     & 33.95 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Celebrity}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 83.60 \\
% 2    & Blip2                     & 81.67 \\
% 3    & InstructBlip              & 75.94 \\
% 4    & Qwen-VL                   & 60.43 \\
% 5    & Shikra-VQA                & 58.61 \\
% 6    & LLAVA-1.5-13B             & 56.20 \\
% 7    & Shikra                    & 56.08 \\
% 8    & MiniGPT-4                 & 46.70 \\
% 9    & LLAVA-1.5-7B              & 45.20 \\
% 10   & Otter                     & 38.39 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Food}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 82.18 \\
% 2    & Blip2                     & 82.16 \\
% 3    & InstructBlip              & 74.20 \\
% 4    & Qwen-VL                   & 60.29 \\
% 5    & Shikra                    & 54.03 \\
% 6    & LLAVA-1.5-13B             & 53.77 \\
% 7    & Shikra-VQA                & 52.86 \\
% 8    & MiniGPT-4                 & 46.45 \\
% 9    & LLAVA-1.5-7B              & 42.07 \\
% 10   & Otter                     & 39.52 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Plant}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 60.37 \\
% 2    & LLAVA-1.5-7B              & 42.53 \\
% 3    & Blip2                     & 42.20 \\
% 4    & LLAVA-1.5-13B             & 41.30 \\
% 5    & MiniGPT-4                 & 39.18 \\
% 6    & Shikra                    & 38.98 \\
% 7    & Qwen-VL                   & 37.56 \\
% 8    & Shikra-VQA                & 37.47 \\
% 9    & InstructBlip              & 35.75 \\
% 10   & Otter                     & 32.18 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Age}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Blip2                     & 93.97 \\
% 2    & InstructBlip              & 80.44 \\
% 3    & XComposer-VL              & 79.56 \\
% 4    & LLAVA-1.5-13B             & 74.03 \\
% 5    & Shikra-VQA                & 63.62 \\
% 6    & Shikra                    & 62.06 \\
% 7    & Qwen-VL                   & 56.05 \\
% 8    & MiniGPT-4                 & 51.87 \\
% 9    & LLAVA-1.5-7B              & 51.33 \\
% 10   & Otter                     & 39.31 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Gender}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 78.59 \\
% 2    & Blip2                     & 67.94 \\
% 3    & InstructBlip              & 67.72 \\
% 4    & Shikra-VQA                & 65.00 \\
% 5    & Shikra                    & 61.51 \\
% 6    & Qwen-VL                   & 59.16 \\
% 7    & LLAVA-1.5-13B             & 58.33 \\
% 8    & LLAVA-1.5-7B              & 53.00 \\
% 9    & MiniGPT-4                 & 45.37 \\
% 10   & Otter                     & 39.91 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Expression}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 62.21 \\
% 2    & Blip2                     & 52.98 \\
% 3    & InstructBlip              & 48.42 \\
% 4    & LLAVA-1.5-13B             & 47.80 \\
% 5    & Qwen-VL                   & 44.81 \\
% 6    & Shikra-VQA                & 42.09 \\
% 7    & LLAVA-1.5-7B              & 41.75 \\
% 8    & Shikra                    & 41.07 \\
% 9    & MiniGPT-4                 & 38.03 \\
% 10   & Otter                     & 28.77 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Race}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Blip2                     & 90.07 \\
% 2    & XComposer-VL              & 87.80 \\
% 3    & InstructBlip              & 82.43 \\
% 4    & Qwen-VL                   & 65.20 \\
% 5    & LLAVA-1.5-13B             & 60.13 \\
% 6    & Shikra-VQA                & 55.53 \\
% 7    & Shikra                    & 53.98 \\
% 8    & MiniGPT-4                 & 48.02 \\
% 9    & Otter                     & 46.92 \\
% 10   & LLAVA-1.5-7B              & 44.73 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Animal}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Blip2                     & 83.55 \\
% 2    & XComposer-VL              & 81.03 \\
% 3    & InstructBlip              & 76.06 \\
% 4    & Qwen-VL                   & 61.06 \\
% 5    & LLAVA-1.5-13B             & 56.84 \\
% 6    & Shikra-VQA                & 55.02 \\
% 7    & MiniGPT-4                 & 49.61 \\
% 8    & Shikra                    & 46.96 \\
% 9    & LLAVA-1.5-7B              & 44.26 \\
% 10   & Otter                     & 38.32 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Object}}
% \end{minipage}
% % \vspace{0.1cm}
% % \begin{minipage}[t]{0.22\textwidth}
% %     \vspace{0pt}
% %     \centering
% %     \setlength\tabcolsep{4.0pt}
% %     \resizebox{1\linewidth}{!}{
% %         \begin{tabular}{c|l|c}
% %         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
% %         \Xhline{1.0pt}

% %         \end{tabular}
% %     }
% %     \subcaption{\textit{Pr.Att.-OCR}}
% % \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 60.60 \\
% 2    & Blip2                     & 52.84 \\
% 3    & LLAVA-1.5-13B             & 45.26 \\
% 4    & Qwen-VL                   & 43.55 \\
% 5    & LLAVA-1.5-7B              & 42.23 \\
% 6    & Shikra                    & 41.06 \\
% 7    & MiniGPT-4                 & 40.32 \\
% 8    & Shikra-VQA                & 40.12 \\
% 9    & InstructBlip              & 40.03 \\
% 10   & Otter                     & 33.86 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Style}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 64.99 \\
% 2    & Shikra-VQA                & 55.50 \\
% 3    & Blip2                     & 54.94 \\
% 4    & Shikra                    & 54.16 \\
% 5    & LLAVA-1.5-13B             & 51.16 \\
% 6    & InstructBlip              & 49.98 \\
% 7    & Qwen-VL                   & 49.17 \\
% 8    & LLAVA-1.5-7B              & 44.34 \\
% 9    & MiniGPT-4                 & 39.23 \\
% 10   & Otter                     & 37.94 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Background}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & XComposer-VL              & 78.66 \\
% 2    & Blip2                     & 74.47 \\
% 3    & InstructBlip              & 63.59 \\
% 4    & Qwen-VL                   & 58.40 \\
% 5    & Shikra                    & 51.75 \\
% 6    & Shikra-VQA                & 51.10 \\
% 7    & LLAVA-1.5-13B             & 49.48 \\
% 8    & LLAVA-1.5-7B              & 43.40 \\
% 9    & MiniGPT-4                 & 41.70 \\
% 10   & Otter                     & 35.56 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Pr.Att.-Color}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
 
% \end{minipage}
% \vspace{0.1cm}
% \caption{Leaderboards of all Perceptual tasks under print attacking scenario.}
% \label{leaderboard_print_fine_grain}
% \end{table*}
% % ==================================================================================================================



% \begin{table*}[h]
% \centering
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Qwen-VL                   & 58.17 \\
% 2    & Shikra                    & 57.41 \\
% 3    & Shikra-VQA                & 57.26 \\
% 4    & LLAVA-1.5-13B             & 57.17 \\
% 5    & Otter                     & 56.61 \\
% 6    & LLAVA-1.5-7B              & 51.91 \\
% 7    & MiniGPT-4                 & 36.95 \\
% 8    & Blip2                     & 33.33 \\
% 9    & InstructBlip              & 31.97 \\
% 10   & XComposer-VL              & 31.75 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Movie}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Shikra-VQA                & 85.84 \\
% 2    & Qwen-VL                   & 79.11 \\
% 3    & Shikra                    & 77.17 \\
% 4    & LLAVA-1.5-13B             & 66.37 \\
% 5    & Otter                     & 65.81 \\
% 6    & LLAVA-1.5-7B              & 60.84 \\
% 7    & MiniGPT-4                 & 37.59 \\
% 8    & Blip2                     & 34.64 \\
% 9    & XComposer-VL              & 33.88 \\
% 10   & InstructBlip              & 32.85 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Action}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Qwen-VL                   & 55.79 \\
% 2    & Shikra-VQA                & 53.57 \\
% 3    & Otter                     & 53.05 \\
% 4    & LLAVA-1.5-13B             & 53.03 \\
% 5    & Shikra                    & 52.61 \\
% 6    & LLAVA-1.5-7B              & 48.36 \\
% 7    & MiniGPT-4                 & 38.22 \\
% 8    & XComposer-VL              & 34.45 \\
% 9    & Blip2                     & 32.04 \\
% 10   & InstructBlip              & 30.93 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-TV Show}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Shikra-VQA                & 71.47 \\
% 2    & Shikra                    & 67.66 \\
% 3    & Qwen-VL                   & 64.80 \\
% 4    & Otter                     & 61.44 \\
% 5    & LLAVA-1.5-13B             & 59.83 \\
% 6    & LLAVA-1.5-7B              & 56.15 \\
% 7    & MiniGPT-4                 & 36.95 \\
% 8    & Blip2                     & 36.14 \\
% 9    & InstructBlip              & 35.02 \\
% 10   & XComposer-VL              & 30.86 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Profession}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Shikra-VQA                & 78.40 \\
% 2    & Shikra                    & 77.85 \\
% 3    & Qwen-VL                   & 76.34 \\
% 4    & LLAVA-1.5-13B             & 71.92 \\
% 5    & LLAVA-1.5-7B              & 68.62 \\
% 6    & Otter                     & 56.87 \\
% 7    & MiniGPT-4                 & 35.73 \\
% 8    & XComposer-VL              & 35.33 \\
% 9    & Blip2                     & 34.53 \\
% 10   & InstructBlip              & 32.03 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Landmark}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Qwen-VL                   & 60.07 \\
% 2    & Otter                     & 51.86 \\
% 3    & LLAVA-1.5-13B             & 51.81 \\
% 4    & Shikra-VQA                & 48.45 \\
% 5    & Shikra                    & 47.75 \\
% 6    & LLAVA-1.5-7B              & 47.32 \\
% 7    & MiniGPT-4                 & 38.38 \\
% 8    & Blip2                     & 37.95 \\
% 9    & InstructBlip              & 34.29 \\
% 10   & XComposer-VL              & 30.89 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Anime}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Qwen-VL                   & 69.92 \\
% 2    & Shikra-VQA                & 68.32 \\
% 3    & Shikra                    & 65.73 \\
% 4    & LLAVA-1.5-13B             & 58.83 \\
% 5    & Otter                     & 57.58 \\
% 6    & LLAVA-1.5-7B              & 47.05 \\
% 7    & MiniGPT-4                 & 38.05 \\
% 8    & InstructBlip              & 36.65 \\
% 9    & XComposer-VL              & 36.41 \\
% 10   & Blip2                     & 36.18 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Clothes}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Qwen-VL                   & 64.77 \\
% 2    & Shikra                    & 60.02 \\
% 3    & Shikra-VQA                & 59.70 \\
% 4    & LLAVA-1.5-13B             & 55.53 \\
% 5    & LLAVA-1.5-7B              & 54.95 \\
% 6    & Otter                     & 52.26 \\
% 7    & MiniGPT-4                 & 37.48 \\
% 8    & Blip2                     & 34.72 \\
% 9    & InstructBlip              & 33.52 \\
% 10   & XComposer-VL              & 33.09 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Celebrity}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Shikra-VQA                & 75.26 \\
% 2    & Qwen-VL                   & 73.72 \\
% 3    & Shikra                    & 71.07 \\
% 4    & LLAVA-1.5-13B             & 64.95 \\
% 5    & Otter                     & 64.39 \\
% 6    & LLAVA-1.5-7B              & 52.30 \\
% 7    & MiniGPT-4                 & 36.94 \\
% 8    & XComposer-VL              & 33.16 \\
% 9    & Blip2                     & 32.48 \\
% 10   & InstructBlip              & 32.13 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Food}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Qwen-VL                   & 79.59 \\
% 2    & Shikra-VQA                & 76.06 \\
% 3    & Shikra                    & 73.53 \\
% 4    & Otter                     & 67.16 \\
% 5    & LLAVA-1.5-13B             & 64.44 \\
% 6    & LLAVA-1.5-7B              & 47.41 \\
% 7    & MiniGPT-4                 & 37.74 \\
% 8    & Blip2                     & 35.84 \\
% 9    & InstructBlip              & 34.02 \\
% 10   & XComposer-VL              & 34.00 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Plant}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Shikra                    & 56.95 \\
% 2    & Shikra-VQA                & 56.80 \\
% 3    & LLAVA-1.5-13B             & 51.43 \\
% 4    & Qwen-VL                   & 48.11 \\
% 5    & LLAVA-1.5-7B              & 45.89 \\
% 6    & Otter                     & 42.82 \\
% 7    & MiniGPT-4                 & 37.14 \\
% 8    & Blip2                     & 34.16 \\
% 9    & InstructBlip              & 33.14 \\
% 10   & XComposer-VL              & 30.78 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Age}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & LLAVA-1.5-13B             & 89.35 \\
% 2    & Shikra-VQA                & 89.06 \\
% 3    & Shikra                    & 85.34 \\
% 4    & Otter                     & 82.25 \\
% 5    & Qwen-VL                   & 79.18 \\
% 6    & LLAVA-1.5-7B              & 51.95 \\
% 7    & MiniGPT-4                 & 48.38 \\
% 8    & Blip2                     & 39.48 \\
% 9    & InstructBlip              & 38.51 \\
% 10   & XComposer-VL              & 38.09 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Gender}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Shikra-VQA                & 82.04 \\
% 2    & Shikra                    & 79.86 \\
% 3    & Qwen-VL                   & 73.91 \\
% 4    & LLAVA-1.5-13B             & 63.13 \\
% 5    & Otter                     & 60.44 \\
% 6    & LLAVA-1.5-7B              & 55.70 \\
% 7    & MiniGPT-4                 & 41.07 \\
% 8    & Blip2                     & 35.95 \\
% 9    & InstructBlip              & 33.52 \\
% 10   & XComposer-VL              & 32.80 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Expression}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & LLAVA-1.5-13B             & 63.06 \\
% 2    & Shikra-VQA                & 61.19 \\
% 3    & Shikra                    & 60.24 \\
% 4    & Qwen-VL                   & 59.50 \\
% 5    & LLAVA-1.5-7B              & 45.97 \\
% 6    & Otter                     & 45.50 \\
% 7    & MiniGPT-4                 & 37.47 \\
% 8    & Blip2                     & 36.81 \\
% 9    & InstructBlip              & 36.36 \\
% 10   & XComposer-VL              & 34.77 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Race}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Qwen-VL                   & 81.78 \\
% 2    & Shikra-VQA                & 80.44 \\
% 3    & Otter                     & 78.00 \\
% 4    & Shikra                    & 77.66 \\
% 5    & LLAVA-1.5-13B             & 70.94 \\
% 6    & LLAVA-1.5-7B              & 49.30 \\
% 7    & MiniGPT-4                 & 37.61 \\
% 8    & Blip2                     & 35.23 \\
% 9    & XComposer-VL              & 34.38 \\
% 10   & InstructBlip              & 34.01 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Animal}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Shikra-VQA                & 79.05 \\
% 2    & Qwen-VL                   & 77.26 \\
% 3    & Shikra                    & 69.98 \\
% 4    & LLAVA-1.5-13B             & 65.33 \\
% 5    & Otter                     & 62.69 \\
% 6    & LLAVA-1.5-7B              & 52.62 \\
% 7    & MiniGPT-4                 & 37.84 \\
% 8    & Blip2                     & 37.62 \\
% 9    & XComposer-VL              & 36.97 \\
% 10   & InstructBlip              & 36.88 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Object}}
% \end{minipage}
% \vspace{0.1cm}
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Shikra-VQA                & 79.12 \\
% 2    & Shikra                    & 77.62 \\
% 3    & Qwen-VL                   & 76.50 \\
% 4    & Otter                     & 74.91 \\
% 5    & LLAVA-1.5-13B             & 66.43 \\
% 6    & XComposer-VL              & 53.21 \\
% 7    & InstructBlip              & 50.03 \\
% 8    & Blip2                     & 47.80 \\
% 9    & LLAVA-1.5-7B              & 46.78 \\
% 10   & MiniGPT-4                 & 36.78 \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-OCR}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Qwen-VL                   & 56.80 \\
% 2    & Otter                     & 53.47 \\
% 3    & Shikra                    & 51.05 \\
% 4    & Shikra-VQA                & 50.30 \\
% 5    & LLAVA-1.5-13B             & 50.01 \\
% 6    & LLAVA-1.5-7B              & 44.85 \\
% 7    & MiniGPT-4                 & 37.98 \\
% 8    & XComposer-VL              & 37.20 \\
% 9    & InstructBlip              & 36.20 \\
% 10   & Blip2                     & 35.87 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Style}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Shikra-VQA                & 65.41 \\
% 2    & Shikra                    & 64.50 \\
% 3    & Otter                     & 60.30 \\
% 4    & Qwen-VL                   & 60.09 \\
% 5    & LLAVA-1.5-13B             & 56.28 \\
% 6    & LLAVA-1.5-7B              & 46.53 \\
% 7    & MiniGPT-4                 & 36.91 \\
% 8    & Blip2                     & 35.05 \\
% 9    & XComposer-VL              & 34.71 \\
% 10   & InstructBlip              & 34.45 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Background}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
% 1    & Qwen-VL                   & 69.63 \\
% 2    & Shikra                    & 69.57 \\
% 3    & Shikra-VQA                & 69.05 \\
% 4    & LLAVA-1.5-13B             & 54.28 \\
% 5    & Otter                     & 53.12 \\
% 6    & LLAVA-1.5-7B              & 46.08 \\
% 7    & MiniGPT-4                 & 37.54 \\
% 8    & XComposer-VL              & 37.23 \\
% 9    & Blip2                     & 36.83 \\
% 10   & InstructBlip              & 35.81 \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Ad.Att.-Color}}
% \end{minipage}
% \vspace{0.1cm}
% \caption{Leaderboards of all Perceptual tasks under adversarial attacking scenario.}
% \label{leaderboard_adver_fine_grain}
% \end{table*}













% % ===========================================================================================
% \begin{table*}[h]
% \centering
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}

%    1    & XComposer-VL& 72.37
% \\
% 2    & InstructBlip& 67.41
% \\
% 3    & Blip2& 66.13
% \\
% 4    & Qwen-VL-Chat& 62.68
% \\
% 5    & Shikra& 62.52
% \\
% 6    & LLAVA-1.5-13B& 59.28
% \\
% 7    & Shikra-VQA& 58.64
% \\
% 8    & Otter& 55.49
% \\
% 9    & LLAVA-1.5-7B& 51.75
% \\
% 10   & MiniGPT-4& 42.64
% \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Clean}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL& 71.63
% \\
% 2    & InstructBlip& 67.62
% \\
% 3    & Blip2& 65.49
% \\
% 4    & Shikra& 62.37
% \\
% 5    & Qwen-VL-Chat& 60.58
% \\
% 6    & LLAVA-1.5-13B& 58.73
% \\
% 7    & Shikra-VQA& 58.47
% \\
% 8    & Otter& 55.42
% \\
% 9    & LLAVA-1.5-7B& 46.44
% \\
% 10   & MiniGPT-4& 42.87
% \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Corru.}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & XComposer-VL& 63.75
% \\
% 2    & Blip2& 56.20
% \\
% 3    & Qwen-VL-Chat & 51.57
% \\
% 4    & InstructBlip& 51.23
% \\
% 5    & LLAVA-1.5-13B& 50.70
% \\
% 6    & Shikra& 49.08
% \\
% 7    & LLAVA-1.5-7B& 46.47
% \\
% 8    & Shikra-VQA& 43.72
% \\
% 9    & MiniGPT-4& 42.87
% \\
% 10   & Otter&  47.10
% \\

%         \end{tabular}
%     }
%     \subcaption{\textit{Print Attack}}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.22\textwidth}
%     \vspace{0pt}
%     \centering
%     \setlength\tabcolsep{4.0pt}
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{c|l|c}
%         \textbf{Rank} & \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\textit{Score}} \\
%         \Xhline{1.0pt}
%         1    & Qwen-VL-Chat& 60.39
%         \\
%         2    & Shikra& 59.31
%         \\
%         3    & LLAVA-1.5-13B& 56.84
%         \\
%         4    & Shikra-VQA& 55.16
%         \\
%         5    & Otter& 51.94
%         \\
%         6    & LLAVA-1.5-7B& 50.07
%         \\
%         7    & InstructBlip& 33.13
%         \\
%         8    & MiniGPT-4& 32.95
%         \\
%         9    & Blip2& 32.65
%         \\
%         10   & XComposer-VL&  30.52
%         \\
%         \end{tabular}
%     }
%     \subcaption{\textit{Adversarial Attack}}
% \end{minipage}
% \vspace{0.1cm}
% \caption{Leaderboards of comprehensive performance in clean, corruption, print attack and adversarial attack scenario.}
% \label{leaderboard_comprehensive}
% \end{table*}
